Route to Time and Time to Route: Travel Time Estimation from Sparse Trajectories

Due to the rapid development of Internet of Things (IoT) technologies, many online web apps (e.g., Google Map and Uber) estimate the travel time of trajectory data collected by mobile devices. However, in reality, complex factors, such as network communication and energy constraints, make multiple trajectories collected at a low sampling rate. In this case, this paper aims to resolve the problem of travel time estimation (TTE) and route recovery in sparse scenarios, which often leads to the uncertain label of travel time and route between continuously sampled GPS points. We formulate this problem as an inexact supervision problem in which the training data has coarsely grained labels and jointly solve the tasks of TTE and route recovery. And we argue that both two tasks are complementary to each other in the model-learning procedure and hold such a relation: more precise travel time can lead to better inference for routes, in turn, resulting in a more accurate time estimation). Based on this assumption, we propose an EM algorithm to alternatively estimate the travel time of inferred route through weak supervision in E step and retrieve the route based on estimated travel time in M step for sparse trajectories. We conducted experiments on three real-world trajectory datasets and demonstrated the effectiveness of the proposed method.

==> Formulation.tex <==

Given a sequence of road segments, estimating the travel time is to produce the total time cost. But as we mentioned, in sparse scenario, the route and the label of each road segment become uncertainty, since we only know the total time cost $T$ between $p_a$ and $p_b$. \figref{fig:data_gens} illustrates the data generating process with  graphical representation. Given $p_a$ and $p_b$, we firstly infer the 
most possible route $r$. $X_{1:K}$\footnote{The subscript for example $X_{1:K}$ denotes an abbreviation for the set $\{X_1,X_2,\cdots,X_K\}$} stand for the features of road segment (e.g., road types, road lanes) in route $r= \{e_1, e_2, \cdots , e_K \}$, where $e_i$ is the $i$th road segment. $Z_i$ denotes the unobservable  \textit{true target travel time} at $e_i$ generating by averaging all trajectories pass time with high-sampling rate in specific time interval.
In this paper, we assume each latent variable $Z_i$ belong to the Lognormal distribution $Z_i \sim \frac{1}{z \sigma \sqrt{2 \pi}} \exp \left(-\frac{(\ln z -\mu)^{2}}{2 \sigma^{2}}\right)$, which has been demonstrated that well performance in fitting real life travel time distribution \cite{pu2011analytic,rakha2006estimating}. The conditional probability could equivalence with
$P(Z_i \mid \theta )=P(Z_i \mid (\mu,\sigma)=f(X;W))$, where $W$ and $X$ are the co-factors to generate the parameterized $\theta$ by the  deterministic function $f$. $W$ is the collection of all weight parameters. The $T$ is the observations of total travel time between $p_a$ and $p_b$ and can be observed via an aggregate function $Q$ with $T=Q(Z_{1:K})=\sum_{i=1}^{K}Z_i$. Here, we summarize two basic assumption used in our paper.
%Noted that the travel time of each road also can be defined as the latent variable. However, due to we can't reach the driver current status, such as,  waiting, wandering or worry, travel time contains multiple uncertainty and large 
%variance. Travel speed $V$ and travel time $T$ are the \textit{aggregate  observation} from $Z$ through the \textit{aggregate functions} $Q: Z^K\rightarrow V, H:Z^K\rightarrow T$. $Z$ under a parametric distribution $p(Z|\theta)$. $W$ and $X$ are the co-factors to generate the parameterized $\theta$ by the  deterministic function $f$ with $\theta=f(X;W)$.  
%\begin{definition}\label{def:speed}
%	Given a sequence of road $R=\{r_1,r_2 \cdots r_K\}$ under two consecutive GPS points in trajectory and it's unobserved travel speed $Z=\{\tilde{v}_1,\tilde{v}_2 \cdots \tilde{v}_K\}$. The aggregate functions $Q$ and $H$ could be defined as 
%	\begin{align}
%		Q(Z)=\frac{\sum^{K}_{i} l_i a_i \tilde{v}_i}{\sum_j^{K} l_j a_j}, \quad H(Z)=\frac{\sum^{K}_{i} l_i a_i }{Q(Z)},
%	\end{align}
%where the calculate average speed formula $Q$ is based on the widely assumption that  the average speed along a path  is given by a length weighted average of speeds over road segments \cite{li2015inferring,li2019learning,wu2016probabilistic}.
%\end{definition}

\noindent\textbf{Assumption 1} \textit{(Aggregate observation assumption)} $p(T \mid X_{1:K}, Z_{1:K}) = p(T \mid Z_{1:K})$

\textit{We assume that the observation $T$ is conditionally dependent with $X_{1:K}$ when given $Z_{1:K}$. This assumption is uniformed with existing studies \cite{carbonneau2018multiple} and conformed to the TTE problem, since given $Z$, the observation $T$ can be determined by  aggregate function $Q$.}

\begin{figure}
	\centering
	\tikz[line width=1pt]{
		% nodes
		\node[obs] (x) {$X$};%
		\node[obs, left = of x, xshift=-0.2cm, yshift=0.5cm] (pa) {$p_a$};%
		\node[obs, left = of x, xshift=-0.2cm, yshift=-0.5cm] (pb) {$p_b$};%
		\node[latent, right = of x, xshift=0.2cm] (z) {$Z$};%
		\node[obs, right = of z, xshift=0.2cm,yshift=-0.0cm] (t) {$T$};%
		\node[latent, above = 10mm of z] (w) {$W$};%
		\edge {w,x} {z}
		\edge {z} {t}
		\edge {pa,pb} {x}
		% plate
		\plate [inner sep=2.5mm, xshift=-0.2cm, yshift=0.1cm] {plate1} {(x)(z)} {$K$ roads segments}; %
		\plate [inner sep=1.0mm, xshift=-0.0cm] {plate1} {(x)(z)(t)(pa)(pb)} {$N$ points}; %
	}
	\caption{ The graphical model of the data generating process. The grey and while node represent the observation and hidden variable respectively.
	}\label{fig:data_gens}
\end{figure}
\noindent\textbf{Assumption 2} \textit{(Markov chain assumption)} $p(Z_{1: K} \mid X_{1: K}) \allowbreak =p(Z_{1} \mid X_{1})\prod_{i=2}^{K}    p(Z_{i+1}   \mid X_{i+1}; Z_{i})$

\textit{We assume that $Z_{i+1}$ are mutually independent except for $Z_{i}$ . This is under the assumption of Markov chain  and extensive applications in trajectory data mining \cite{brakatsoulas2005map,li2015inferring}. Further, since  $T$ can be determined by function $Q$, the conditional probability can be defined as $p(T\mid Z_{1: K})=\delta_{T\left(Z_{1: K}\right)}(T)$, where $\delta(\cdot)$ represents the \textit{Dirac delta function}.}



%Due to the $V$ and $T$ are equivalent when travel distance is given (\defref{def:speed}),  we consider to maximizes the conditional probability of travel average speed $V$, since $V$ is always under the reasonable interval $\left[0 kph, 180 kph \right]$ compared with travel time $T$. Therefore, the conditional distribution $p\left(V \mid X_{1: K}\right)$ could be written as
%\begin{align}
%	\max \nonumber ~&p\left(V \mid X_{1: K}\right)\\ \nonumber
%	=&\int_{Z^{K}}p\left(V; Z_{1: K} \mid X_{1: K}\right)\\\nonumber
%	=&\int_{Z^{K}} \delta_{Q\left(z_{1: K}\right)}(V) 
%	p(Z_{1} \mid X_{1})\prod_{i=2}^{K}   \allowbreak p(Z_{i+1}   \mid X_{i}; Z_{i})\nonumber \\
%	=&\underset{Z_{i} \sim p\left(Z_{i} \mid X_{i}\right)}{\mathbb{E}}\left[\delta_{Q\left(Z_{1: K}\right)}(V) \right]
%%	&=\mathbb{E}\left[\log p\left(S;T \mid X_{1: K} ; W\right)\right]
%\end{align}
%Since $V$ and $X_{1: K}$ are the observe variable, we use the  learnable parameter $W$ to maximize the probability $p\left(V \mid X_{1: K}\right)$, which can be defined as \textit{ expected log-likelihood} \cite{zhang2020learning}
%\begin{align}
%	\ell(W)=\mathbb{E}\left[\log p\left(Y \mid X_{1: K} ; W\right)\right]\label{equ:obj}
%\end{align}

Consequently, the objective function in this paper can be written as
\begin{align}\label{eqn:obj}
	 \arg \max_{X_{1:K}, W} \log P(T \mid X_{1:K}; W).
\end{align}

Subsequently, we derive the \eqnref{eqn:obj} through EM algorithm, which  heuristically divided the training process into  expectation (E step) and maximization (M step).

E step:
\begin{align}
&\mathbb{E}\left[\log P(T \mid X_{1:K})\mid T^{(i)}; X_{1:K}^{(i)}; W^{(i)} \right]
\nonumber\\
=&\int_{Z^{K}} \log P(T\mid Z_{1:K}; X_{1:K}) P(Z_{1:K}\mid X_{1:K}) d_{Z_{1:K}} \nonumber\\
=&\int_{Z^{K}} \delta_{Q\left(z_{1: K}\right)}(T) 
p(Z_{1} \mid X_{1})\prod_{i=2}^{K}   \allowbreak p(Z_{i+1}   \mid X_{i+1}; Z_{i})d_{Z_{1:K}} \nonumber \\
=&\underset{Z_{i} \sim p\left(Z_{i} \mid X_{i}; Z_{i-1}\right)}{\mathbb{E}}\left[\delta_{Q\left(Z_{1: K}\right)}(T) \right]\label{eqn:weakly}
\end{align}

M step:
\begin{align}
	\widehat{X}_{1:K}&=\arg \max_{X_{1:K}} \log P(T \mid X_{1:K}; p_a; p_b; W)\label{eqn:search}
\end{align}

The expectation item aims to estimate the travel time distribution of each road segment by weakly supervised learning, and the maximization item unfolds the routes through heuristically searching. After that, the final travel time of trajectory $Tr: p_{1} \rightarrow p_{2} \rightarrow \cdots \rightarrow p_{|T r|}$ can be obtained by summing all estimating components $\Theta=\{ \widetilde{T}_1,\widetilde{T}_2, \cdots, \widetilde{T}_{|Tr|-1} \}$ between any continuous GPS samples with $\widetilde{T}=\sum_{i=1}^{|Tr|-1} \widetilde{T}_i$. Finally, our task can be described that given the current time $\mathbf{t}$, we assume the  traffic conditions at a specific time interval $\Delta \mathbf{t}$ (e.g., 30 minutes) are temporally invariant and train the trajectories to those within the time slot $[\mathbf{t},\mathbf{t}+  \frac{\mathbf{\Delta t}}{2})$. The estimating traffic conditions will be evaluated by using the trajectories in $[\mathbf{t}+  \frac{\mathbf{\Delta t}}{2},\mathbf{t}+ \Delta \mathbf{t})$.  



